Human to Document, AI to Code: Comparing GenAI for Notebook Competitions

Computational notebooks have become the preferred tool of choice for data scientists and practitioners to perform analyses and share results. Notebooks uniquely combine scripts with documentation. With the emergence of generative AI (GenAI) technologies, it is increasingly important, especially in competitive settings, to distinguish the characteristics of human-written versus GenAI. In this study, we present three case studies to explore potential strengths of both humans and GenAI through the coding and documenting activities in notebooks. We first characterize differences between 25 code and documentation features in human-written, medal-winning Kaggle notebooks. We find that gold medalists are primarily distinguished by longer and more detailed documentation. Second, we analyze the distinctions between human-written and GenAI notebooks. Our results show that while GenAI notebooks tend to achieve higher code quality (as measured by metrics like code smells and technical debt), human-written notebooks display greater structural diversity, complexity, and innovative approaches to problem-solving. Based on these results, we envision the work as groundwork that highlight four agendas to further investigate how GenAI could be utilized in notebooks that maximizes the potential collaboration between human and AI.

==> figures/RQ1-dist-markdown-cell.tex <==
\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{figures/pdf/gold_nongold_markdown_cell.pdf}
    \centering
    \caption{Distribution of \#Markdown Cell.}
    \label{fig:RQ1-Dist-Markdown-Cell}
\end{figure}

==> figures/RQ1-dist-markdown-char.tex <==
\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{figures/pdf/gold_nongold_markdown_char.pdf}
    \centering
    \caption{Distribution of \#Markdown Char.}
    \label{fig:RQ1-Dist-Markdown-Char}
\end{figure}

==> figures/RQ1-dist-markdown-line.tex <==
\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{figures/pdf/gold_nongold_markdown_line.pdf}
    \centering
    \caption{Distribution of \#Markdown Line.}
    \label{fig:RQ1-Dist-Markdown-Line}
\end{figure}

==> figures/RQ1-dist-sentence.tex <==
\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{figures/pdf/gold_nongold_sentence.pdf}
    \centering
    \caption{Distribution of Sentence.}
    \label{fig:RQ1-Dist-Markdown-Sentence}
\end{figure}

==> figures/dist-medal.tex <==
\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{figures/pdf/dist_medal.pdf}
    \centering
    \caption{Distribution of Medal Across Competition.}
    \label{fig:dist-medal}
\end{figure}

==> tables/ai-gold.tex <==

% Define colors for effect size highlighting
\definecolor{negligible}{RGB}{240,248,255}
\definecolor{small}{RGB}{173,216,230}
\definecolor{medium}{RGB}{100,149,237}
\definecolor{large}{RGB}{65,105,225}

\begin{table}[htbp]
\centering
\caption{Statistical Comparisons of AI and Gold
Medal Notebooks}
\label{tab:ai-gold}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|>{\centering\arraybackslash}p{1.2cm}>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.2cm}>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.2cm}>{\centering\arraybackslash}p{1.2cm}}
\toprule
& \multicolumn{2}{c|}{\textbf{Home-Credit}} & \multicolumn{2}{c|}{\textbf{Santander}} & \multicolumn{2}{c}{\textbf{IEEE-CIS}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(l){6-7}
\textbf{Feature} & p-value & effect size & p-value & effect size & p-value & effect size \\
\midrule
Functions & \textbf{0.011*} & \cellcolor{large}\textbf{0.197} & - & - & \textbf{0.041*} & \cellcolor{medium}0.078 \\
Statements & \textbf{0.025*} & \cellcolor{large}\textbf{0.143} & - & - & - & - \\
Comment Lines & \textbf{0.035*} & \cellcolor{medium}0.122 & - & - & - & - \\
\#Code Cell & \textbf{0.049*} & \cellcolor{medium}0.103 & - & - & \textbf{0.025*} & \cellcolor{medium}0.098 \\
Cyclomatic Complexity & \textbf{0.050*} & \cellcolor{medium}0.102 & - & - & - & - \\
Gunning Fog & - & - & \textbf{0.017*} & \cellcolor{medium}0.124 & \textbf{0.032*} & \cellcolor{medium}0.088 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ai-human-stats-all.tex <==

% Define colors for alternating rows
\definecolor{lightblue}{RGB}{240,248,255}
\definecolor{mediumblue}{RGB}{173,216,230}

\begin{table}[htbp]
\centering
\caption{AI vs Human Feature Statistics Comparison in IEEE-CIS Competition}
\label{tab:ai-human-stats}
\resizebox{\columnwidth}{2.8cm}{%
\begin{tabular}{ll|l|c|c|c|c|c}
\hline
\textbf{Competition} & \textbf{Feature} & \textbf{Source} & \textbf{Mean} & \textbf{Median} & \textbf{Std} & \textbf{Min} & \textbf{Max} \\
\hline
\multirow{14}{*}{Home-Credit} & \multirow{2}{*}{Functions} & Human & 5.71 & 3.0 & 6.41 & 0 & 29 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}4.00 & \cellcolor{lightblue}1.0 & \cellcolor{lightblue}6.08 & \cellcolor{lightblue}0 & \cellcolor{lightblue}11 \\
\cline{2-8}
 & \multirow{2}{*}{Statements} & Human & 194.38 & 151.5 & 164.06 & 0 & 720 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}144.33 & \cellcolor{lightblue}65.0 & \cellcolor{lightblue}178.73 & \cellcolor{lightblue}19 & \cellcolor{lightblue}349 \\
\cline{2-8}
 & \multirow{2}{*}{Comment Lines} & Human & 66.93 & 44.0 & 70.36 & 0 & 366 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}43.67 & \cellcolor{lightblue}25.0 & \cellcolor{lightblue}49.70 & \cellcolor{lightblue}6 & \cellcolor{lightblue}100 \\
\cline{2-8}
 & \multirow{2}{*}{\#Code Cell} & Human & 33.65 & 21.0 & 45.65 & 1 & 475 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}13.00 & \cellcolor{lightblue}14.0 & \cellcolor{lightblue}5.57 & \cellcolor{lightblue}7 & \cellcolor{lightblue}18 \\
\cline{2-8}
 & \multirow{2}{*}{Cyclomatic Complexity} & Human & 18.53 & 12.5 & 23.07 & 0 & 167 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}16.00 & \cellcolor{lightblue}6.0 & \cellcolor{lightblue}22.72 & \cellcolor{lightblue}0 & \cellcolor{lightblue}42 \\
\cline{2-8}
 & \multirow{2}{*}{Gunning Fog} & Human & 11.13 & 10.22 & 8.12 & 0.00 & 46.99 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}8.47 & \cellcolor{lightblue}11.71 & \cellcolor{lightblue}7.40 & \cellcolor{lightblue}0.00 & \cellcolor{lightblue}13.7 \\
\cline{2-8}
 & \multirow{2}{*}{Code Smells} & Human & 140.36 & 1.0 & 838.82 & 0 & 8582 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}1.33 & \cellcolor{lightblue}1.0 & \cellcolor{lightblue}1.53 & \cellcolor{lightblue}0 & \cellcolor{lightblue}3 \\
\cline{2-8}
 & \multirow{2}{*}{Technical Depts} & Human & 165.87 & 5.0 & 850.56 & 0 & 8694 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}10.67 & \cellcolor{lightblue}5.0 & \cellcolor{lightblue}14.36 & \cellcolor{lightblue}0 & \cellcolor{lightblue}27 \\
\cline{2-8}
 & \multirow{2}{*}{Violations} & Human & 140.84 & 1.0 & 839.49 & 0 & 8590 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}1.33 & \cellcolor{lightblue}1.0 & \cellcolor{lightblue}1.53 & \cellcolor{lightblue}0 & \cellcolor{lightblue}3 \\
\hline
\multirow{18}{*}{Santander} & \multirow{2}{*}{Functions} & Human & 2.48 & 1.0 & 4.19 & 0 & 23 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}0.00 & \cellcolor{lightblue}0.0 & \cellcolor{lightblue}0.00 & \cellcolor{lightblue}0 & \cellcolor{lightblue}0 \\
\cline{2-8}
 & \multirow{2}{*}{Statements} & Human & 93.59 & 67.0 & 94.96 & 0 & 602 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}56.00 & \cellcolor{lightblue}29.0 & \cellcolor{lightblue}51.16 & \cellcolor{lightblue}24 & \cellcolor{lightblue}115 \\
\cline{2-8}
 & \multirow{2}{*}{Comment Lines} & Human & 30.99 & 14.0 & 43.04 & 0 & 298 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}20.67 & \cellcolor{lightblue}15.0 & \cellcolor{lightblue}12.50 & \cellcolor{lightblue}12 & \cellcolor{lightblue}35 \\
\cline{2-8}
 & \multirow{2}{*}{\#Code Cell} & Human & 18.17 & 14.0 & 13.88 & 0 & 69 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}9.00 & \cellcolor{lightblue}7.0 & \cellcolor{lightblue}3.46 & \cellcolor{lightblue}7 & \cellcolor{lightblue}13 \\
\cline{2-8}
 & \multirow{2}{*}{Cyclomatic Complexity} & Human & 9.95 & 6.0 & 12.43 & 0 & 59 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}0.67 & \cellcolor{lightblue}0.0 & \cellcolor{lightblue}1.15 & \cellcolor{lightblue}0 & \cellcolor{lightblue}2 \\
\cline{2-8}
 & \multirow{2}{*}{Gunning Fog} & Human & 10.46 & 10.12 & 7.31 & 0 & 54.4 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}17.13 & \cellcolor{lightblue}18.88 & \cellcolor{lightblue}3.70 & \cellcolor{lightblue}12.88 & \cellcolor{lightblue}19.63 \\
\cline{2-8}
 & \multirow{2}{*}{Code Smells} & Human & 2.68 & 0.0 & 5.78 & 0 & 41 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}0.67 & \cellcolor{lightblue}1.0 & \cellcolor{lightblue}0.58 & \cellcolor{lightblue}0 & \cellcolor{lightblue}1 \\
\cline{2-8}
 & \multirow{2}{*}{Technical Depts} & Human & 15.14 & 0.0 & 36.51 & 0 & 320 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}3.33 & \cellcolor{lightblue}5.0 & \cellcolor{lightblue}2.89 & \cellcolor{lightblue}0 & \cellcolor{lightblue}5 \\
\cline{2-8}
 & \multirow{2}{*}{Violations} & Human & 3.01 & 0.0 & 6.36 & 0 & 49 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}0.67 & \cellcolor{lightblue}1.0 & \cellcolor{lightblue}0.58 & \cellcolor{lightblue}0 & \cellcolor{lightblue}1 \\
\hline
\multirow{18}{*}{IEEE-CIS} & \multirow{2}{*}{Functions} & Human & 3.16 & 2.0 & 5.99 & 0 & 46 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}0.67 & \cellcolor{lightblue}0.0 & \cellcolor{lightblue}1.15 & \cellcolor{lightblue}0 & \cellcolor{lightblue}2 \\
\cline{2-8}
 & \multirow{2}{*}{Statements} & Human & 121.49 & 91.5 & 112.14 & 10 & 586 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}94.33 & \cellcolor{lightblue}35.0 & \cellcolor{lightblue}111.54 & \cellcolor{lightblue}25 & \cellcolor{lightblue}223 \\
\cline{2-8}
 & \multirow{2}{*}{Comment Lines} & Human & 40.93 & 23.5 & 49.54 & 0 & 252 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}32.67 & \cellcolor{lightblue}18.0 & \cellcolor{lightblue}29.84 & \cellcolor{lightblue}13 & \cellcolor{lightblue}67 \\
\cline{2-8}
 & \multirow{2}{*}{\#Code Cell} & Human & 31.36 & 22.0 & 32.82 & 2 & 205 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}9.00 & \cellcolor{lightblue}8.0 & \cellcolor{lightblue}2.65 & \cellcolor{lightblue}7 & \cellcolor{lightblue}12 \\
\cline{2-8}
 & \multirow{2}{*}{Cyclomatic Complexity} & Human & 14.30 & 9.5 & 17.53 & 0 & 126 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}14.67 & \cellcolor{lightblue}0.0 & \cellcolor{lightblue}25.40 & \cellcolor{lightblue}0 & \cellcolor{lightblue}44 \\
\cline{2-8}
 & \multirow{2}{*}{Gunning Fog} & Human & 10.32 & 9.91 & 7.99 & 0 & 64.61 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}16.07 & \cellcolor{lightblue}16.13 & \cellcolor{lightblue}4.49 & \cellcolor{lightblue}11.55 & \cellcolor{lightblue}20.53 \\
\cline{2-8}
 & \multirow{2}{*}{Code Smells} & Human & 29.25 & 0.0 & 264.35 & 0 & 3166 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}3.00 & \cellcolor{lightblue}3.0 & \cellcolor{lightblue}0.00 & \cellcolor{lightblue}3 & \cellcolor{lightblue}3 \\
\cline{2-8}
 & \multirow{2}{*}{Technical Depts} & Human & 44.39 & 0.0 & 272.18 & 0 & 3228 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}15.00 & \cellcolor{lightblue}15.0 & \cellcolor{lightblue}0.00 & \cellcolor{lightblue}15 & \cellcolor{lightblue}15 \\
\cline{2-8}
 & \multirow{2}{*}{Violations} & Human & 29.59 & 0.0 & 264.45 & 0 & 3167 \\
 &  & \cellcolor{lightblue}AI & \cellcolor{lightblue}3.00 & \cellcolor{lightblue}3.0 & \cellcolor{lightblue}0.00 & \cellcolor{lightblue}3 & \cellcolor{lightblue}3 \\
\hline
\end{tabular}
}
\end{table}

==> tables/ai-nongold.tex <==
% Define colors for effect size highlighting
\definecolor{negligible}{RGB}{240,248,255}
\definecolor{small}{RGB}{173,216,230}
\definecolor{medium}{RGB}{100,149,237}
\definecolor{large}{RGB}{65,105,225}

\begin{table}[htbp]
\centering
\caption{Statistical Comparisons of AI and Non-Gold Medal
Notebooks}
\label{tab:ai-nongold}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|>{\centering\arraybackslash}p{1.2cm}>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.2cm}>{\centering\arraybackslash}p{1.2cm}|>{\centering\arraybackslash}p{1.2cm}>{\centering\arraybackslash}p{1.2cm}}
\toprule
& \multicolumn{2}{c|}{\textbf{Home-Credit}} & \multicolumn{2}{c|}{\textbf{Santander}} & \multicolumn{2}{c}{\textbf{IEEE-CIS}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(l){6-7}
\textbf{Feature} & p-value & effect size & p-value & effect size & p-value & effect size \\
\midrule
Functions & \textbf{0.012*} & \cellcolor{small}0.050 & - & - & - & - \\
Cyclomatic Complexity & \textbf{0.038*} & \cellcolor{small}0.031 & - & - & - & - \\
Statements & \textbf{0.047*} & \cellcolor{small}0.027 & - & - & - & - \\
Gunning Fog & - & - & \textbf{0.032*} & \cellcolor{small}0.027 & \textbf{0.040*} & \cellcolor{small}0.026 \\
Code Smells & - & - & - & - & \textbf{0.034*} & \cellcolor{small}0.028 \\
Technical Depts & - & - & - & - & \textbf{0.039*} & \cellcolor{small}0.026 \\
\bottomrule
\end{tabular}
}
\end{table}

\vspace{1em}

